VL-SAE: Interpreting and Enhancing Vision-Language Alignment with a Unified Concept Set

The alignment of vision-language representations endows current Vision-Language Models (VLMs) with strong multi-modal reasoning capabilities. However, the interpretability of the alignment component remains uninvestigated due to the difficulty in mapping the semantics of multi-modal representations into a unified concept set. To address this problem, we propose VL-SAE, a sparse autoencoder that encodes vision-language representations into its hidden activations. Each neuron in its hidden layer correlates to a concept represented by semantically similar images and texts, thereby interpreting these representations with a unified concept set. To establish the neuron-concept correlation, we encourage semantically similar representations to exhibit consistent neuron activations during self-supervised training. First, to measure the semantic similarity of multi-modal representations, we perform their alignment in an explicit form based on cosine similarity. Second, we construct the VL-SAE with a distance-based encoder and two modality-specific decoders to ensure the activation consistency of semantically similar representations. Experiments across multiple VLMs (e.g., CLIP, LLaVA) demonstrate the superior capability of VL-SAE in interpreting and enhancing the vision-language alignment. For interpretation, the alignment between vision and language representations can be understood by comparing their semantics with concepts. For enhancement, the alignment can be strengthened by aligning vision-language representations at the concept level, contributing to performance improvements in downstream tasks, including zero-shot image classification and hallucination elimination. Codes are available at https://github.com/ssfgunner/VL-SAE.

==> Styles/tables/app_data_volume.tex <==
\begin{table}[]
\centering
\caption{Concept Quality of VL-SAE trained with different proportions of the CC3M dataset.}
\begin{tabular}{@{}cccccc@{}}
\toprule
Data Percentage      & 10\%   & 30\%   & 50\%   & 70\%   & 100\%  \\ \midrule
Intra-Similarity~($\uparrow$) & 0.2029 & 0.2129 & 0.2196 & 0.2222 & 0.2299 \\
Inter-Similarity~($\downarrow$) & 0.1597 & 0.1306 & 0.126  & 0.1256 & 0.1220 \\ \bottomrule
\end{tabular}
\label{tab: app_data_volume}
\end{table}

==> Styles/tables/app_topk.tex <==
\begin{table}[]
\centering
\caption{Ablation studies of the sparsification method in VL-SAE.}
\begin{tabular}{@{}ccc@{}}
\toprule
Method & Intra-Similarity~($\uparrow$) & Inter-Similarity~($\downarrow$) \\ \midrule
L1     & 0.2142           & 0.1809           \\
Top-K  & \textbf{0.2442}           & \textbf{0.1373}           \\ \bottomrule
\end{tabular}
\label{tab: app_topk}
\end{table}
